Tuneful: An Online Significance-Aware Configuration Tuner for Big Data Analytics

Distributed analytics engines such as Spark are a common choice for processing extremely large datasets. However, finding good configurations for these systems remains challenging, with each workload potentially requiring a different setup to run optimally. Using suboptimal configurations incurs significant extra runtime costs. %Furthermore, Spark and similar platforms are gaining traction within data-scientists communities where awareness of such issues is relatively low. We propose Tuneful, an approach that efficiently tunes the configuration of in-memory cluster computing systems. Tuneful combines incremental Sensitivity Analysis and Bayesian optimization to identify near-optimal configurations from a high-dimensional search space, using a small number of executions. This setup allows the tuning to be done online, without any previous training. Our experimental results show that Tuneful reduces the search time for finding close-to-optimal configurations by 62\% (at the median) when compared to existing state-of-the-art techniques. This means that the amortization of the tuning cost happens significantly faster, enabling practical tuning for new classes of workloads.

==> 040-challenges.tex <==

%\begin{figure} [t]
%	%\centering
%	\hspace{-5mm}
%	\includegraphics[height=4cm,width=\columnwidth]{img/sig_params_motivation_2.png}
%	\caption{Relative configuration parameter importance for 3 Hibench workloads, showing that the parameters which affect runtime the most are workload-specific.}
%	\label{fig2}
%\end{figure}

%In this section we discuss the challenges associated with tuning the configuration of analytic workloads.

\noindgras{Number of Samples}:
The search space for good configurations grows exponentially with the number of configuration parameters.
Spark~\cite{spark} has over 180 configuration parameters. Not all of them impact performance, but some of the relevant ones have large intervals of possible values.

For example, the search space of three Spark configuration parameters (\ie memory per executor, cores per executer and spark memory fraction) contains more than 4000 combinations, assuming a cluster of nodes with 60 GB memory and 16 processing cores.
%Executing a workload can take several dozen hours~%\cite{kannan2016seesaw},
An exhaustive search can represent thousands of hours of wasted computational power and associated monetary cost.
Therefore, it is crucial to minimize the number of configurations evaluated to reach an optimal configuration.


\noindgras{No single configuration fits all workloads:}
Each workload has particular characteristics in terms of resource usage,
(\eg some workloads are CPU intensive, while others are memory or shuffle heavy).
Therefore there is no one single optimal configuration, but instead workload-specific optimal configurations that are a function of workload characteristics, including the distribution and size of input data.
Moreover, the configuration parameters that have the biggest impact on the runtime also vary depending on the workload characteristics.
~\autoref{fig2} depicts the significant configuration parameters for three workloads from Hibench~\cite{hibench}: Pagerank and two Bayesian classifiers with different input sizes.

The calculation of the significance is based on the contribution of each configuration parameter in predicting the execution time, as determined from 100 executions of each workload. As expected, for each of these workloads, the set of significant configuration parameters is different.

\noindgras{Frequent Workload changes:}
A change in a workload takes place either through modifying the execution logic
or through a significant change of the processed data size (\eg new records need analysis).
While the former is rare in a deployed system, the later is common in the big data world.
For example, consider a Pagerank workload, initially processing a dataset of 5 million pages. Running daily and receiving roughly 100K pages of additional data at each run, the dataset grows to 14m pages in 3 months (90 executions of the workload). Such changes can lead to significant changes in the workload's behaviour under particular configurations, as shown in~\autoref{fig1}. 

The configuration should therefore be re-tuned accordingly. While the decision about \emph{when} to re-tune is independent from the tuning strategy, its feasibility relies on how expensive is to re-run tuning in the setting of gradually changing workloads. 

Existing approaches for high-dimensional configuration tuning require a significant number of executions for finding close-to-optimal solutions. In particular, the number of executions required generally exceeds the number of times the workload might run before re-tuning is necessary.
For example, the \texttt{BestConfig}~\cite{bestconfig} system requires hundreds of samples to identify a good configuration, so the convergence to optimal might not happen during the 90 ``normal'' runs of our example workload over the 3 months period. Furthermore, exploring the configuration space will inevitably lead to some suboptimal execution times, and the associated cost is difficult to amortize in few or no optimal executions.

==> 090-fw.tex <==
%\notetp{Discuss limitations openly here.
%This is a proof of concept.
%Our next objective is to perform a deployment at scale.
%Maybe discuss exploring AWS/Google/Microsoft instances as exploration domain.}

%Tuneful is an efficient approach for self tuning data analytics systems.
%Here, we discuss its limitations and our future directions.
%Tuneful is implemented as a proof of concept, we are refactoring the code to release it as an open-source extension to Spark. \notetp{I though that was already done?}
%Currently Tuneful explores the configurations related to the Spark level of parallelism and its performance surpasses prior work. 
%We are planning to extend Tuneful exploration to other configuration parameters in the hope to reduce workload execution time even further.
%We are not expecting adding more configuration parameters to significantly influence Tuneful effectiveness, as some recent work has been proposed to enable High-dimensional GP optimization~\cite{djolonga2013high,duvenaud2011additive}. 
%Additionally, we are keen to experiment with constrained multi-objective optimization (\eg minimizing energy consumption and execution latency while maintaining expenses below a certain level).
%We plan to move from a proof of concept to a more realistic deployment and are looking for partners to explore opportunity on platforms such as AWS, Google  EC2 and Microsoft Azure.
%Finally, the approach adopted by Tuneful has application beyond Spark.
%We plan to explore the approach proposed here in scenarios such as cloud configuration tuning~\cite{cherrypick} and VM selection~\cite{paris}.


==> ack.tex <==
%We thank Clayton Crabideau for inspring this work through troubleshooting his PDB preprocessing workload on Spark. 
%We also thank Thomas Bytheway for his valuable comments, which certainly helped in shaping the final version of the paper.
%This work is funded by the Egyptian Ministry of Higher Education and Cambridge Trust.


==> availability.tex <==
This work has been open-sourced under license Apache 2.0 open-source and is available online at \emph{anonymised}.
